Authenticating On-Body Backscatter by Exploiting Propagation Signatures

The vision of battery-free communication has made backscatter a compelling technology for on-body wearable and implantable devices. Recent advances have facilitated the communication between backscatter tags and on-body smart devices. These studies have focused on the communication dimension, while the security dimension remains vulnerable. It has been demonstrated that wireless connectivity can be exploited to send unauthorized commands or fake messages that result in device malfunctioning. The key challenge in defending these attacks stems from the minimalist design in backscatter. Thus, in this paper, we explore the feasibility of authenticating an on-body backscatter tag without modifying its signal or protocol. We present SecureScatter, a physical-layer solution that delegates the security of backscatter to an on-body smart device. To this end, we profile the on-body propagation paths of backscatter links, and construct highly sensitive propagation signatures to identify on-body backscatter links. We implement our design in a software radio and evaluate it with different backscatter tags that work at 2.4 GHz and 900 MHz. Results show that our system can identify on-body devices at 93.23% average true positive rate and 3.18% average false positive rate.

==> background.tex <==
%!TEX root=main.tex
\section{Preliminary}
\label{sec_pre}
In this section, we briefly introduce the operating mechanism of human breath and intrinsic reasons why deep breathing can be leveraged for liveness detection to enhance the security level of heart sound authentication.

\subsection{Breathing Mechanism}
Breathing is the process of gas exchange between the human body and the environment, which brings in oxygen and flushes out carbon dioxide. There are two phases of normal breathing: \emph{inhalation}(or \emph{inspiration}) and \emph{exhalation}(or \emph{expiration}). Many organs are involved in breathing, including nose, trachea, lungs, rib cage, muscles and diaphragm. During inhalation, the diaphragm(a large sheet of muscle under the lungs) and the intercostal muscles will contract to pull the rib cage upwards and bulge the abdomen out. Such a process extends the volume of the chest cavity, and lowers the pressure in the lung. At the same time, fresh air would pass through the nasal or mouth cavity and trachea, and eventually arrives at the lung. Exhalation is the reverse process of inhalation: the diaphragm and intercostal muscles relax so that the rib cage and abdomen return to their origin position, when the waste air will be flushed out of the body.\cite{Breathing}. 

% Breathing repeat iteratively to sustain the life. 

Deep breathing, as a special form of breathing, is distinct from normal breathing in the following aspects. First, normal breathing is involuntary and imperceptible by people in most cases, while deep breathing generally occurs due to intended actions by people. 
Second, in deep breathing, abdomen muscles involve much more actively during inspiration so that the diaphragm is the main engine to drive deep breathing \cite{diaphragmaticbreathing}. Third, the movement of the diaphragm and rib cage will be to larger degree in deep breathing than that in normal breathing, thus a larger volume of air will be exchanged in deep breathing.

% different from normal breath involves the expansion of the chest during inspiration, deep breath involves the expansion of the both chest and belly which lead to the motion of diaphragm becomes the dominate\cite{diaphragmaticbreathing}. 

\subsection{Breathing Sound and Chest Movement}
\label{sec_soundandmotion}
Medical researchers have investigated breathing sounds and chest movement for decades. Chest movement caused by muscle and rib cage movement can be measured by inertial sensors\cite{sumbul2015measuring} on the chest to monitor the respiration cycle\cite{bates2010respiratory} and detect sleep apnea\cite{nandakumar2015contactless}. Inertial readings of the chest were revealed to be highly correlated with airflow waveform generated in breathing\cite{bates2010respiratory}, because the intensity of chest movement has a direct effect on the volume and rate of airflow. In deep breathing, when the diaphragm, abdomen muscles and rib cage jointly change the pressure of the chest cavity and lung to a larger degree, more and faster airflow goes through the trachea and lungs. The larger airflow rate then produces a louder breathing sound. Many theories(linear\cite{kraman1984relationship}, cube\cite{yosef2009effect}) have been proposed to model and explain the high correlation between airflow rate and breathing sound\cite{goel2016spirocall}. However, the exact relationship between breathing sound and airflow in the respiratory system have not been firmly established. 

Breathing characteristics vary across different people due to age\cite{gross2000relationship} and gender\cite{gross2000relationship}. Besides, for the same person, breathing characteristics vary across different times during a short term\cite{vlemincx2013respiratory} due to different muscle status, emotions\cite{boiten1994emotions} and environment\cite{Breathing}. Thus, deep breathing has a randomness property beneficial to liveness detection.

The above analysis of deep breathing provides the following insights for our system:
\begin{enumerate}
\item The degree of chest movement highly correlates to the intensity of breathing sound. In our target scenarios, people wear chest straps/bands to monitor heart rate/heart sound for fitness. Thus, we leverage the chest-worn setting, and utilize a chest-mounted MEMS gyroscope and microphone on the traditional auscultation site to measure the movement of the chest(diaphragm, rib cage) and record breathing sounds respectively. 
\item The exact relationship between breathing motion and breathing sound depends on the complicated structure of the individual respiratory system. Thus, it is difficult to infer the exact breathing motion from breathing sounds and vice versa, which significantly reduces the possibility of an attack. 
\item Breathing characteristics not only vary across people but also  different breaths from the same person, which makes precise deep breathing imitation even harder for attackers. 
\end{enumerate}



==> implementation.tex <==
%!TEX root=main.tex

\section{Implementation}
\label{sec_implementation}
In this section, we illustrate how we build BreathLive prototype.  

The system contains the following parts: arduino boards, amplifier, microphone, motion sensor and stethoscope diaphragm. Fig.~\ref{hardware} shows the hardware composition of our system. The stethoscope diaphragm is a plastic disc mounted on a metal head, which can be vibrated by body sounds if placed on the surface of the skin. A motion sensor MPU6050 Six-Axis(Gyrosocpe + Accelerometer) and an Electret microphone are used to capture signals. The former is attached on the surface of the stethoscope to capture chest movement, and the latter is placed inside the stethoscope to capture the sound. Since body sounds are rather low compared to other ambient sounds, we use Max9812, a low-cost 20dB fixed-gain microphone amplifier. To capture both signals with enough sampling rates, two Arduino Uno boards collect data from two sensors respectively. Arduino Uno is a microcontroller board based on the 16MHz ATmega328 with multiple digital pins and analog inputs. The amplified sound signal will be captured by the analog pin of Arduino 1 with the sampling rate of 7800Hz, which is high enough to capture the heart sound and lung sound. MPU6050 communicates with Arduino 2 through I2C communication protocol at the sampling rate of 350Hz. To minimize the delay between the two signals, a synchronization line would be set to trigger Arduino 2, when Arduino 1 begins data sampling. However, due to the imperfection manufactures of crystal oscillators on two Arduinos, the delay can only be reduced but not totally removed. That is the reason why synchronization is needed in our algorithm. A Windows 10 laptop will communicate with two Arduinos simultaneously and analyze the data off-line. 

Fig. \ref{prototype} shows the BreathLive prototype, and Fig. \ref{realuse} shows the real usage scenario of chest-worn monitor wearables. The prototype can be fixed on the body using a strap. In the enrollment phase, the user needs to train the model by doing a few deep breaths. The system trains the classifier based on not only the data from this user but also from pre-restored data from other users.  Then the system can function well to detect whether the current access is a live person or a pretender with pre-recorded sound.


\begin{figure}
\begin{minipage}[t]{0.48\textwidth}
\centering
\includegraphics[width=1\textwidth]{Implementation1}
\caption{The hardware diagram of BreathLive.\ } 
\label{hardware}
\end{minipage}
\hspace{1.5ex}
\begin{minipage}[t]{0.48\textwidth}
\centering
\includegraphics[width=0.9\textwidth]{prototype}
\caption{The real prototype of our system. It is exactly the same structure as the hardware diagram shows.}
\label{prototype} 
\end{minipage}
\end{figure}

\begin{figure}
\begin{minipage}[t]{0.2\textwidth}
\centering
\includegraphics[width=1\textwidth]{realuse1}

\end{minipage}
\hspace{20ex}
\begin{minipage}[t]{0.2\textwidth}
\centering
\includegraphics[width=1\textwidth]{realuse2}
\end{minipage}
\caption{The typical user scenario of our system. The left-hand figure shows the device worn on the chest. The right-hand figure shows the approximate position on the rib cage and near the diaphragm. In practical usage, the device should be worn inside the clothes to capture a high quality signal. It is reasonable because most of the chest worn wearables on the market need to contact the skin.}
\label{realuse} 
\end{figure}
